A Flexible Patch-Based Lattice Boltzmann Parallelization Approach for Heterogeneous GPU-CPU Clusters

Sustaining a large fraction of single GPU performance in parallel computations is considered to be the major problem of GPU-based clusters. In this article, this topic is addressed in the context of a lattice Boltzmann flow solver that is integrated in the WaLBerla software framework. We propose a multi-GPU implementation using a block-structured MPI parallelization, suitable for load balancing and heterogeneous computations on CPUs and GPUs. The overhead required for multi-GPU simulations is discussed in detail and it is demonstrated that the kernel performance can be sustained to a large extent. With our GPU implementation, we achieve nearly perfect weak scalability on InfiniBand clusters. However, in strong scaling scenarios multi-GPUs make less efficient use of the hardware than IBM BG/P and x86 clusters. Hence, a cost analysis must determine the best course of action for a particular simulation task. Additionally, weak scaling results of heterogeneous simulations conducted on CPUs and GPUs simultaneously are presented using clusters equipped with varying node configurations.

==> Hybrid-Algorithm.tex <==
%===========================================================
%
% Author:           $Author: unrz55 $
% Date of Commit:   $Date: 2010/07/07 12:54:40 $
% Tag Name:         $Name: ARXIV $
% Revision:         $Revision: 1.1 $
% Source path:      $Source: /opt/cvsrep/SC-GPU-2010/arXiv/Hybrid-Algorithm.tex,v $
%===========================================================

\section{Homogeneous and Heterogeneous parallelization Strategies}
%
%


